Re-designing Dynamic Content Delivery in the Light of a Virtualized Infrastructure

We explore the opportunities and design options enabled by novel SDN and NFV technologies, by re-designing a dynamic Content Delivery Network (CDN) service. Our system, named MOSTO, provides performance levels comparable to that of a regular CDN, but does not require the deployment of a large distributed infrastructure. In the process of designing the system, we identify relevant functions that could be integrated in the future Internet infrastructure. Such functions greatly simplify the design and effectiveness of services such as MOSTO. We demonstrate our system using a mixture of simulation, emulation, testbed experiments and by realizing a proof-of-concept deployment in a planet-wide commercial cloud system.

==> references.tex <==
The impact of brokers on the future of content delivery
    Content delivery is performed putting together several CDNs. Smaller specialized CDNs are joining the market leveraging the brokers to get customers.

Trimming the smartphone network stack
    offload the network stack to the base station for energy saving.
    
The Internet at the speed of light
    It reports that TCP slow start is a major source of latency
    Good for introduction/motivation.
    
    There are also some considerations about using ALEXA
    
Demystifying Page Load Performance with WProf
    They show the different contributions to page load time, doing measurements with both HTTP and SPDY.
    An interesting result is that Page Load TIme is affected by those components that are on the critical load path. Because of that, caching may only partially help.
    In particular, caching only helps when cached objects are on the critical path. 
    
Measuring and Mitigating Web Performance Bottlenecks in Broadband Access Networks
    The paper measures the performance of loading 9 popular web pages from >5k locations. They highlight the importance of latency and also have importance considerations about last mile latencies. 
    The paper starting from this observations makes a point about having a form of caching happening already in the home routers. The benefits are already available in the caching of DNS and TCP connections.
    Another important observation is that sites performance largely depends from the availability of CDN sites in the geographical area, and that even larger CDNs do not completely cover all the areas.
    
Web content cartography
    They envision an important role for virtualization in future CDNs.

Mapping the Expansion of Google's Serving Infrastructure
    The paper shows that google has expanded its network using satellites nodes deployed very close to the edge. Apparently they do it to improve connections with split-TCP.
    - Could we use miniproxy-like solutions to push back the need for satellites? Or to make those deployments more democratic?
    
A Server-to-Server view of the Internet
    Presents latency results coming from measurements between Akamai's servers. Results: congestion is not the norm in the network's core. When congestion happens, up to 20ms increase in RTT. Route changes happen infrequently and mostly do not affect the server-to-server RTT

End-User Mapping: next generation request routing for content delivery
    The paper presentes the AKamai's request routing system that instructs the local DNS resolvers. THe paper presents the results of the rollout of the system. It also motivates why few tens of ms are an important optimization. The need to scale the system handling DNS requests is also discussed, since a more precise user's mapping requires more frequent DNS interactions.
